Leveraging edge detection and neural networks for better UAV localization

We propose a novel method for geolocalizing Unmanned Aerial Vehicles (UAVs) in environments lacking Global Navigation Satellite Systems (GNSS). Current state-of-the-art techniques employ an offline-trained encoder to generate a vector representation (embedding) of the UAV's current view, which is then compared with pre-computed embeddings of geo-referenced images to determine the UAV's position. Here, we demonstrate that the performance of these methods can be significantly enhanced by preprocessing the images to extract their edges, which exhibit robustness to seasonal and illumination variations. Furthermore, we establish that utilizing edges enhances resilience to orientation and altitude inaccuracies. Additionally, we introduce a confidence criterion for localization. Our findings are substantiated through synthetic experiments.

==> Makefile <==
#PDF  = $(shell ls *.tex | sed 's/\.tex/.pdf/')

#all : $(PDF)
all : main-igarss.pdf

%.pdf : %.tex ; cat $< | bash pdflatexfilter > $@

clean : ; $(RM) $(PDF)

